Learning Monocular Dense Depth from Events

Event cameras are novel sensors that output brightness changes in the form of a stream of asynchronous events instead of intensity frames. Compared to conventional image sensors, they offer significant advantages: high temporal resolution, high dynamic range, no motion blur, and much lower bandwidth. Recently, learning-based approaches have been applied to event-based data, thus unlocking their potential and making significant progress in a variety of tasks, such as monocular depth prediction. Most existing approaches use standard feed-forward architectures to generate network predictions, which do not leverage the temporal consistency presents in the event stream. We propose a recurrent architecture to solve this task and show significant improvement over standard feed-forward methods. In particular, our method generates dense depth predictions using a monocular setup, which has not been shown previously. We pretrain our model using a new dataset containing events and depth maps recorded in the CARLA simulator. We test our method on the Multi Vehicle Stereo Event Camera Dataset (MVSEC). Quantitative experiments show up to 50% improvement in average depth error with respect to previous event-based methods.

==> chapters/sup.tex <==
\section{Why using events for Depth prediction?}
\label{sec:appendixb}

\begin{figure*}[t!]
    \centering
    $\begin{array}{cc}
    \subcaptionbox{\label{fig:tunnel_frame} Frame}
    {
        \includegraphics[width=0.5\textwidth,keepaspectratio]{images/results/morning_tunnel_davis_0000000637}
    }
    \hspace{-0.1cm}
    \subcaptionbox{\label{fig:tunnel_megadepth} MegaDepth on frames~\cite{Li18cvpr}}
    {
        \includegraphics[width=0.5\textwidth,keepaspectratio]{images/results/morning_tunnel_megadepth_0000000637}
    }
    \end{array}$
    $\begin{array}{cc}
    \hspace{-0.1cm}
    \subcaptionbox{\label{fig:tunnel_events} Events}
    {
        \includegraphics[width=0.5\textwidth,keepaspectratio]{images/results/morning_tunnel_events_white_0000000637}
    }
    \hspace{-0.1cm}
    \subcaptionbox{\label{fig:tunnel_prediction} Ours on events}
    {
        \includegraphics[width=0.5\textwidth,keepaspectratio]{images/results/morning_tunnel_prediction_0000000637}
    }
    \end{array}$
    \caption{Qualitative results in a high dynamic range (HDR)  situation facing the
    sun when driving a car on a highway.~\ref{fig:tunnel_frame} grayscale frame from
    a DAVIS camera.~\ref{fig:tunnel_megadepth} Depth prediction from
    MegaDepth.~\ref{fig:tunnel_events} Events and~\ref{fig:tunnel_prediction} our depth map prediction using events}
   \label{fig:tunnel_result}
\end{figure*}

\begin{figure*}[t!]
    \centering
    $\begin{array}{cc}
    \subcaptionbox{\label{fig:e2vid} E2VID\cite{Rebecq19pami}}
    {
        \includegraphics[width=0.5\textwidth,keepaspectratio]{images/results/e2vid/e2vid_0000001731}
    }
    \hspace{-0.12cm}
    \subcaptionbox{\label{fig:megadepth_e2vid} MegaDepth on E2VID}
    {
        \includegraphics[width=0.5\textwidth,keepaspectratio]{images/results/e2vid/megadepth_e2vid_0000001731}
    }
    \end{array}$
    $\begin{array}{cc}
    \hspace{-0.12cm}
    \subcaptionbox{\label{fig:qualitative_events} Events}
    {
        \includegraphics[width=0.5\textwidth,keepaspectratio]{images/results/e2vid/events_white_0000001731}
    }
    \hspace{-0.12cm}
    \subcaptionbox{\label{fig:qualitative_prediction} Ours on events}
    {
        \includegraphics[width=0.5\textwidth,keepaspectratio]{images/results/e2vid/prediction_0000001731}
    }
    \end{array}$
    \caption{Qualitative results comparing depth prediction using MegaDepth on reconstructed
    frames from E2VID and our method using events.}
   \label{fig:e2vid_comparison}
\end{figure*}

State of the art research in computer vision has demonstrated that salient edges
and texture are more relevant than color to estimate depth~\cite{huiccv19}.
Event cameras capture salient edges as well as detailed changes in brightness
with high temporal-spatial resolution. This makes event cameras suitable sensors
to predict depth.  We present two qualitative cases in this Appendix.
Fig.~\ref{fig:tunnel_result} shows a comparison by estimating depth from events
in an HDR scenario. Our method predicts depth directly from events while MegaDepth
uses the greyscale frame. MegaDepth shows difficulties to mask the sky due to
overexposure while the prediction from events better approximates the structure
of the scene. However, our method has some difficulties to predict the truck on
the right side of the image. This is because our DENSE dataset and
the~\textit{outdoor day2} sequence from MVSEC do not have moving trucks, so the
network has never seen such a situation during training.
Fig.~\ref{fig:e2vid_comparison} depicts the case of predicting depth from a
reconstructed frame using E2VID~\cite{Rebecq19pami}, which has HDR and does not
suffer from motion blur. The reconstruction shows that depth prediction directly
from events has more level of detail than from a reconstructed frame.


